GM-NeRF: Learning Generalizable Model-based Neural Radiance Fields from Multi-view Images

In this work, we focus on synthesizing high-fidelity novel view images for arbitrary human performers, given a set of sparse multi-view images. It is a challenging task due to the large variation among articulated body poses and heavy self-occlusions. To alleviate this, we introduce an effective generalizable framework Generalizable Model-based Neural Radiance Fields (GM-NeRF) to synthesize free-viewpoint images. Specifically, we propose a geometry-guided attention mechanism to register the appearance code from multi-view 2D images to a geometry proxy which can alleviate the misalignment between inaccurate geometry prior and pixel space. On top of that, we further conduct neural rendering and partial gradient backpropagation for efficient perceptual supervision and improvement of the perceptual quality of synthesis. To evaluate our method, we conduct experiments on synthesized datasets THuman2.0 and Multi-garment, and real-world datasets Genebody and ZJUMocap. The results demonstrate that our approach outperforms state-of-the-art methods in terms of novel view synthesis and geometric reconstruction.

==> tables/ablation_on_noise.tex <==
\begin{table}[ht]
	\centering
	\scalebox{0.75}{
	%\resizebox{\linewidth}{!}{
		\begin{tabular}{c|cccccc}
			\toprule
			Noise $\tau$(cm) & 0 & 1 & 3 & 5 & 10 \\
			\midrule
			
			PSNR$\uparrow$ & 30.12  & 29.14 & 28.58 & 28.19 & 27.09 \\
			
			SSIM$\uparrow$ & 0.9365 & 0.9302 & 0.9243 & 0.9206  & 0.8959 \\
                LPIPS$\downarrow$ & 0.0374 & 0.0462 & 0.0532 & 0.0566 & 0.0729 \\
			\bottomrule
	\end{tabular}}
	\caption{{\bf The impact of different SMPL noise levels.} By adding Gaussian noise (with variance $\tau$) to the SMPL vertices, the performance increases as the noise decreases.}
    \label{tab:ablation_on_noise}
\end{table}

==> tables/ablation_on_views.tex <==
\begin{table}[ht]
	\centering
	\scalebox{0.85}{
	%\resizebox{\linewidth}{!}{
		\begin{tabular}{c|ccc}
			\toprule
			Input views & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
			\midrule
			
			1 & 27.36 & 0.9281 & 0.04854 \\
			
			2 & 29.25 & 0.9393 & 0.03689 \\
			
			4(Ours) & 30.18 & 0.9472 & 0.03049 \\
			
			6 & 30.65 & 0.9530 & 0.02838 \\
			
			8 & 31.01 & 0.9565 & 0.02663 \\
			
			16 & 31.54 & 0.9605 & 0.02448 \\
			\bottomrule
	\end{tabular}}
	\caption{{\bf The Impact of the number of input views}. }
	\label{tab:albation_on_views}
\end{table}


==> tables/image_extraction.tex <==
\begin{table}[ht]
	\centering
	\scalebox{0.75}{
	%\resizebox{\linewidth}{!}{
		\begin{tabular}{l l l}
			\toprule
			
			Layer &\multicolumn{1}{l}{Input (\textbf{ID} :  HWC )} 
			&\multicolumn{1}{c}{Output (\textbf{ID} :  HWC )}
			\\
			\midrule
			
			Conv, 64, k=7, s=2 & \textbf{0} : $512\times 512\times 3$   & \textbf{1} : $256\times 256\times 64$ \\
			Residual layer 1 & \textbf{1} : $256\times 256\times 64$ & \textbf{2} : $256\times 256\times 64$  \\
			
			Residual layer 2 & \textbf{2} : $256\times 256\times 64$ & \textbf{3} : $128\times 128\times 128$  \\

                Residual layer 3 & \textbf{3} : $128\times 128\times 128$ & \textbf{4} : $64\times 64\times 256$  \\
			
			 Upconv, 128, k=3, f=2 & \textbf{4} : $64\times 64\times 256$ & \textbf{5} : $128\times 128\times 128$  \\
			
			 iConv, 128, k=3, s=1 & \textbf{3 © 5}: $128\times 128\times 256$  & \textbf{6} : $128\times 128\times 128$  \\

                Upconv, 64, k=3, f=2 & \textbf{6} : $128\times 128\times 128$ & \textbf{7} : $256\times 256\times 64$  \\

                iConv, 64, k=3, s=1 & \textbf{2 © 7}: $256\times 256\times 128$  & \textbf{8} : $256\times 256\times 64$  \\

                iConv, 64, k=3, s=1 & \textbf{1 © 8}: $256\times 256\times 128$  & \textbf{9} : $256\times 256\times 64$  \\

                Conv, 64, k=1, s=1 & \textbf{9} : $256\times 256\times 64$  & \textbf{10} : $256\times 256\times 64$  \\

			\bottomrule
	\end{tabular}}
	% \vspace{-0.5em}
	\caption{{\bf Image feature extraction network}.  'Conv' stands
for a sequence of operations: convolution (k is kernal size and s is stride), rectified linear units
(ReLU) and Batch Normalization\cite{BN}. 'iConv' replace the Batch Normalization with Instance Normalization\cite{IN} compare with 'Conv'. 'Upconv' stands for a bilinear upsampling with specific factor (f), followed by a 'iConv' operation with stride=1. © represents channel-wise concatenation. 'Residual layer' is the residual blocks of the original ResNet34\cite{ResNet} design,
of two feature maps}
    \vspace{-1em}
	\label{tab:image_extraction}
\end{table}

==> tables/novel_pose_details_on_genebody.tex <==
\begin{table}[ht]
	\centering
	\scalebox{0.75}{
	%\resizebox{\linewidth}{!}{
		\begin{tabular}{c|ccc|ccc}
			\toprule
			
			&\multicolumn{3}{c|}{From Scratch} 
			&\multicolumn{3}{c}{Finetune}
			\\
			\midrule
			
			Model & PNSR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$   & PNSR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
			\midrule
			amanda & 26.45 & 0.947 & 0.0699 & 27.52 & 0.953 & 0.0506 \\
			
			barry & 31.37 & 0.951 & 0.0979 & 32.24 & 0.960 & 0.0456 \\
			
			fuzhizhi & 21.79 & 0.897 & 0.1066 & 22.06 & 0.898 & 0.0995 \\
			
			jinyutong & 21.25 & 0.892 & 0.1215 & 21.97 & 0.899 & 0.1016 \\
			
			joseph & 21.93 & 0.896 & 0.1067 & 24.01 & 0.915 & 0.0803 \\
			
			maria & 20.60 & 0.864 & 0.1449 & 20.62 & 0.862 & 0.1339 \\
			
			manhanran & 30.32 & 0.911 & 0.1485 & 31.46 & 0.942 & 0.0831 \\
			
			natacha & 26.94 & 0.901 & 0.1011 & 27.57 & 0.910 & 0.0764 \\
			
			soufianou & 29.72 & 0.940 & 0.0692 & 30.50 & 0.945 & 0.0541 \\
			
			zhuna & 23.44 & 0.927 & 0.0935 & 23.53 & 0.926 & 0.0845 \\
			\midrule
			Average & 25.38 & 0.912 & 0.1060 & 26.15 & 0.921 & 0.0810 \\
			\bottomrule
	\end{tabular}}
	% \vspace{-0.5em}
	\caption{{\bf Quantitative results on Genebody\cite{genebody} dataset}. }
    \vspace{-1em}
	\label{tab:persence_details_on_genebody}
\end{table}

==> tables/novel_pose_details_on_zjumocap.tex <==
\begin{table}[ht]
	\centering
	\scalebox{0.75}{
	%\resizebox{\linewidth}{!}{
		\begin{tabular}{c|ccc|ccc}
			\toprule
			
			&\multicolumn{3}{c|}{From Scratch} 
			&\multicolumn{3}{c}{Finetune}
			\\
			\midrule
			
			Model & PNSR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$   & PNSR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
			\midrule
			313 & 27.65 & 0.943 & 0.0731 & 28.29 & 0.949 & 0.0622  \\
			
			315 & 25.03 & 0.935 & 0.0858 & 25.68 & 0.944 & 0.0717 \\
			
			377 & 26.49 & 0.930 & 0.0952 & 27.58 & 0.942 & 0.0778 \\
			
			386 & 27.63 & 0.911 & 0.1288 & 29.51 & 0.930 & 0.0983 \\
			
			387 & 24.61 & 0.910 & 0.1084  & 25.59 & 0.926 & 0.0863 \\
			
			390 & 26.86 & 0.916 & 0.1105 & 27.90 & 0.929 & 0.0897 \\
			
			392 & 28.07 & 0.931 & 0.0979 & 28.94 & 0.942 & 0.0788 \\
			
			393 & 26.72 & 0.926 & 0.0883 & 27.54 & 0.938 & 0.0734 \\
			
			394 & 27.04 & 0.916 & 0.0977 & 27.65 & 0.927 & 0.0801 \\
			
			\midrule
			Average & 26.68 & 0.924 & 0.0984 & 27.63 & 0.936 & 0.0798 \\
			\bottomrule
	\end{tabular}}
	% \vspace{-0.5em}
	\caption{{\bf Quantitative results of novel pose synthesis on ZJUMocap\cite{neuralbody} dataset}. }
    % \vspace{-1em}
	\label{tab:novel_pose_details_on_zju_mocap}
\end{table}

==> tables/novel_pose_on_genebody.tex <==
\begin{table}[ht]
	\centering
	\scalebox{0.75}{
	%\resizebox{\linewidth}{!}{
		\begin{tabular}{c|ccc}
			\toprule
			
			&\multicolumn{3}{c}{GeneBody\cite{genebody}} 
			\\
			\midrule
			
			Model & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
			\midrule
			NV\cite{NeuralVolume} & 19.86 & 0.774 &  0.267  \\
			
			NT\cite{NT} & 21.68 & 0.881 &  0.152 \\
			
			NHR\cite{NHR} & 20.05 & 0.800 &  0.155 \\
			
			NB\cite{neuralbody} & 20.73 & 0.878 &  0.231 \\
			
			Ours(Fs) & 25.38 & 0.912 & 0.106  \\
			
			Ours(Ft) & \bf{26.15} & \bf{0.921} & \bf{0.081} \\
			\bottomrule
	\end{tabular}}
	\caption{{\bf Quantitative comparisons on unseen pose with case-specific optimization methods}. We evaluate the novel view synthesis of unseen poses with case-specific optimization methods on GeneBody\cite{genebody}.}
    \label{tab:novel_pose_on_genebody}
\end{table}

==> tables/novel_view_details_on_zjumocap.tex <==
\begin{table}[ht]
	\centering
	\scalebox{0.75}{
	%\resizebox{\linewidth}{!}{
		\begin{tabular}{c|ccc|ccc}
			\toprule
			
			&\multicolumn{3}{c|}{From Scratch} 
			&\multicolumn{3}{c}{Finetune}
			\\
			\midrule
			
			Model & PNSR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$   & PNSR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
			\midrule
			313 & 30.56
 & 0.965 & 0.0532 & 31.49 & 0.971
 & 0.0444 \\
			
			315 & 26.78 & 0.952 & 0.0702 & 26.98 & 0.956 & 0.0607 \\
			
			377 & 27.36 & 0.943 & 0.0775 & 28.38 & 0.952 & 0.0641 \\
			
			386 & 27.50 & 0.914 & 0.1218 & 29.26 & 0.932 & 0.0900 \\
			
			387 & 25.56 & 0.920 &  0.0986 & 26.46 & 0.932 & 0.0804 \\
			
			390 & 26.91 & 0.915 & 0.1070 & 27.73 & 0.926 & 0.0880 \\
			
			392 & 28.54 & 0.929 & 0.0980 & 29.45 & 0.942 & 0.0776 \\
			
			393 & 26.81 & 0.920 & 0.0947 & 27.69 & 0.933 &  0.0785 \\
			
			394 & 28.05 & 0.924 & 0.0923 & 28.64 & 0.934 & 0.0760 \\
			
			\midrule
			Average & 27.56 & 0.931 & 0.0904 & 28.45 & 0.942 & 0.0733 \\
			\bottomrule
	\end{tabular}}
	% \vspace{-0.5em}
	\caption{{\bf Quantitative results of novel view synthesis on ZJUMocap\cite{neuralbody} dataset}. }
	\label{tab:novel_view_details_on_zju_mocap}
\end{table}
